Distilled Lifelong Self-Adaptation for Configurable Systems

Modern configurable systems provide tremendous opportunities for engineering future intelligent software systems. A key difficulty thereof is how to effectively self-adapt the configuration of a running system such that its performance (e.g., runtime and throughput) can be optimized under time-varying workloads. This unfortunately remains unaddressed in existing approaches as they either overlook the available past knowledge or rely on static exploitation of past knowledge without reasoning the usefulness of information when planning for self-adaptation. In this paper, we tackle this challenging problem by proposing DLiSA, a framework that self-adapts configurable systems. DLiSA comes with two properties: firstly, it supports lifelong planning, and thereby the planning process runs continuously throughout the lifetime of the system, allowing dynamic exploitation of the accumulated knowledge for rapid adaptation. Secondly, the planning for a newly emerged workload is boosted via distilled knowledge seeding, in which the knowledge is dynamically purified such that only useful past configurations are seeded when necessary, mitigating misleading information. Extensive experiments suggest that the proposed DLiSA significantly outperforms state-of-the-art approaches, demonstrating a performance improvement of up to 229% and a resource acceleration of up to 2.22x on generating promising adaptation configurations. All data and sources can be found at our repository: https://github.com/ideas-labo/dlisa.

==> macros.tex <==
\usepackage{xspace}


\usepackage{pifont}
\usepackage{pgfplots}
\usepackage{subcaption}
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


\usepackage[all]{nowidow}


\usetikzlibrary{patterns}
\usetikzlibrary{intersections}
\usetikzlibrary{calc}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes.misc}
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand*{\ShowIntersection}[3]{%
    \fill
    [
      name intersections={of=#1 and #2, name=i, total=\t},
    ]
    \foreach \s in {1,...,\t}{(i-\s) circle (2pt)
       node [above #3] {%
        \pgfgetlastxy{\macrox}{\macroy}
        \transformydimension{\macroy}
        \pgfmathprintnumber{\pgfmathresult}}};}  
        
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\aka}{\emph{a.k.a.}\xspace}

\newcommand{\tool}{\textsc{FedDebug}\xspace}
\newcommand{\gulzar}[1]{{\color{red}G: #1}}
\newcommand{\waris}[1]{{\color{green}W: #1}}
\newcommand{\update}[1]{{\color{blue} #1}}
\newcommand{\ali}[1]{{\color{purple}A: #1}}
\newcommand{\todo}[1]{{\color{orange} TODO: #1}}


==> tables/RQ2_efficiency_comparison.tex <==
\small
\footnotesize
%\setlength{\tabcolsep}{1mm}
\setlength{\tabcolsep}{2pt}
		\begin{tabular}{c|cccc|cccc|cccc|cccc}
			\hline
			\multirow{2}{*}{\textbf{System}} & \multicolumn{4}{c|}{\textbf{\textbf{\approach~} vs Pseudo-Dy}}                                                                                          & \multicolumn{4}{c|}{\textbf{\textbf{\approach~} vs LiDOS}}                                                                                              & \multicolumn{4}{c|}{\textbf{\textbf{\approach~} vs Sta-Init}}                                                                                         & \multicolumn{4}{c}{\textbf{\textbf{\approach~} vs D-SOGA}}                                                                                             \\ \cline{2-17} 
			& \multicolumn{1}{c|}{$s$ \textgreater 1} & \multicolumn{1}{c|}{$s$ = 1}       & \multicolumn{1}{c|}{0 \textless $s$ \textless 1} & $s$ = -1      & \multicolumn{1}{c|}{$s$ \textgreater 1} & \multicolumn{1}{c|}{$s$ = 1}       & \multicolumn{1}{c|}{0 \textless $s$ \textless 1} & $s$ = -1      & \multicolumn{1}{c|}{$s$ \textgreater 1} & \multicolumn{1}{c|}{$s$ = 1}      & \multicolumn{1}{c|}{0 \textless $s$ \textless 1} & $s$ = -1     & \multicolumn{1}{c|}{$s$ \textgreater 1} & \multicolumn{1}{c|}{$s$ = 1}      & \multicolumn{1}{c|}{0 \textless $s$ \textless 1} & $s$ = -1      \\ \hline
			\textsc{lrzip}                            & \multicolumn{1}{c|}{5}                & \multicolumn{1}{c|}{6}           & \multicolumn{1}{c|}{0}                         & 2           & \multicolumn{1}{c|}{12}               & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 1           & \multicolumn{1}{c|}{13}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{11}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 2           \\
			\textsc{xz}                               & \multicolumn{1}{c|}{13}               & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{13}               & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{13}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{13}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0           \\
			\textsc{z3}                               & \multicolumn{1}{c|}{3}                & \multicolumn{1}{c|}{4}           & \multicolumn{1}{c|}{0}                         & 5           & \multicolumn{1}{c|}{4}                & \multicolumn{1}{c|}{2}           & \multicolumn{1}{c|}{0}                         & 6           & \multicolumn{1}{c|}{3}                & \multicolumn{1}{c|}{5}          & \multicolumn{1}{c|}{0}                         & 4          & \multicolumn{1}{c|}{3}                & \multicolumn{1}{c|}{1}          & \multicolumn{1}{c|}{0}                         & 8           \\
			\textsc{dconvert}                         & \multicolumn{1}{c|}{1}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 11          & \multicolumn{1}{c|}{1}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 11          & \multicolumn{1}{c|}{12}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{0}                & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 12          \\
			\textsc{batlik}                           & \multicolumn{1}{c|}{1}                & \multicolumn{1}{c|}{1}           & \multicolumn{1}{c|}{0}                         & 9           & \multicolumn{1}{c|}{3}                & \multicolumn{1}{c|}{6}           & \multicolumn{1}{c|}{0}                         & 2           & \multicolumn{1}{c|}{11}               & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{1}                & \multicolumn{1}{c|}{3}          & \multicolumn{1}{c|}{0}                         & 7           \\
			\textsc{kanzi}                            & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0           \\
			\textsc{x264}                             & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{9}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{4}                & \multicolumn{1}{c|}{3}          & \multicolumn{1}{c|}{0}                         & 2          & \multicolumn{1}{c|}{7}                & \multicolumn{1}{c|}{1}          & \multicolumn{1}{c|}{0}                         & 1           \\
			\textsc{h2}                               & \multicolumn{1}{c|}{7}                & \multicolumn{1}{c|}{1}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{7}                & \multicolumn{1}{c|}{1}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{8}                & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{5}                & \multicolumn{1}{c|}{1}          & \multicolumn{1}{c|}{0}                         & 2           \\
			\textsc{jump3r}                           & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{0}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{5}                & \multicolumn{1}{c|}{1}           & \multicolumn{1}{c|}{0}                         & 0           & \multicolumn{1}{c|}{6}                & \multicolumn{1}{c|}{0}          & \multicolumn{1}{c|}{0}                         & 0          & \multicolumn{1}{c|}{4}                & \multicolumn{1}{c|}{2}          & \multicolumn{1}{c|}{0}                         & 0           \\ \hline
			\textbf{Total}                   & \multicolumn{1}{c|}{\textbf{54}}      & \multicolumn{1}{c|}{\textbf{12}} & \multicolumn{1}{c|}{\textbf{0}}                & \textbf{27} & \multicolumn{1}{c|}{\textbf{63}}      & \multicolumn{1}{c|}{\textbf{10}} & \multicolumn{1}{c|}{\textbf{0}}                & \textbf{20} & \multicolumn{1}{c|}{\textbf{79}}      & \multicolumn{1}{c|}{\textbf{8}} & \multicolumn{1}{c|}{\textbf{0}}                & \textbf{6} & \multicolumn{1}{c|}{\textbf{53}}      & \multicolumn{1}{c|}{\textbf{8}} & \multicolumn{1}{c|}{\textbf{0}}                & \textbf{32} \\ \hline
		\end{tabular}

==> tables/RQ3_JUMP3R_ablation_comparison.tex <==

\begin{adjustbox}{max width = 1\columnwidth}
	\begin{tabular}{>{\centering\arraybackslash}p{1.1cm} p{1.4cm}p{1.9cm}p{2.3cm}p{0.8cm}}
		\toprule
		\multicolumn{1}{l}{\textbf{Workload}} & \textbf{Algorithm} & \textbf{Mean (Std)} & \textbf{$\hat{A}_{12}$ ($p$ value)}                          \\ \hline
		& {\approach~}                & 2.599 (0.793)       &                                                              \\
		& {\approach~}-I              & 2.596 (0.612)       & \cellcolor[HTML]{FECDCD}0.547 ($p$ = 0.248)                        \\
		\multirow{-3}{*}{$w_1$}          & {\approach~}-II              & 2.72 (0.778)        & \cellcolor[HTML]{CBFECE}0.576 ($p$ = 0.064)                        \\ \hline
		& {\approach~}                & 0.854 (0.228)       &                                                              \\
		& {\approach~}-I              & 0.888 (0.178)       & \cellcolor[HTML]{CBFECE}\textbf{0.589 ($p$ = 0.029)}               \\
		\multirow{-3}{*}{$w_2$}          & {\approach~}-II              & 0.95 (0.224)        & \cellcolor[HTML]{CBFECE}\textbf{0.649 ($p$ \textless 0.001)} \\ \hline
		& {\approach~}                & 1.295 (0.402)       &                                                              \\
		& {\approach~}-I              & 1.469 (0.475)       & \cellcolor[HTML]{CBFECE}\textbf{0.630 ($p$ = 0.001)}                \\
		\multirow{-3}{*}{$w_3$}          & {\approach~}-II              & 1.544 (0.483)       & \cellcolor[HTML]{CBFECE}\textbf{0.679 ($p$ \textless 0.001)} \\ \hline
		& {\approach~}                & 0.633 (0.089)       &                                                              \\
		& {\approach~}-I              & 0.664 (0.106)       & \cellcolor[HTML]{CBFECE}\textbf{0.612 ($p$ = 0.006)}               \\
		\multirow{-3}{*}{$w_4$}          & {\approach~}-II              & 0.685 (0.118)       & \cellcolor[HTML]{CBFECE}\textbf{0.659 ($p$ \textless 0.001)} \\ \hline
		& {\approach~}                & 1.063 (0.27)        &                                                              \\
		& {\approach~}-I              & 1.195 (0.44)        & \cellcolor[HTML]{CBFECE}\textbf{0.623 ($p$ = 0.003)}               \\
		\multirow{-3}{*}{$w_5$}          & {\approach~}-II              & 1.292 (0.5)         & \cellcolor[HTML]{CBFECE}\textbf{0.647 ($p$ \textless 0.001)} \\ \hline
		& {\approach~}                & 0.296 (0.019)       &                                                              \\
		& {\approach~}-II              & 0.307 (0.026)       & \cellcolor[HTML]{CBFECE}\textbf{0.631 ($p$ = 0.001)}               \\
		\multirow{-3}{*}{$w_6$}          & {\approach~}-II              & 0.309 (0.026)       & \cellcolor[HTML]{CBFECE}\textbf{0.673 ($p$ \textless 0.001)} \\ \hline
	\end{tabular}
\end{adjustbox}

==> tables/RQ4_sensitivity_comparison.tex <==
\resizebox{\textwidth}{!}{ % reSize the table
	\begin{tabular}{p{1.35cm}|p{1.35cm}|p{0.3cm}p{2.0cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{1.95cm}|p{0.3cm}p{2.8cm}|p{0.3cm}p{1.95cm}}
		\hline
		&                                      & \multicolumn{2}{c|}{\textbf{LRZIP}}                                                  & \multicolumn{2}{c|}{\textbf{XZ}}                                                     & \multicolumn{2}{c|}{\textbf{Z3}}                                                    & \multicolumn{2}{c|}{\textbf{DCONVERT}}                                               & \multicolumn{2}{c|}{\textbf{BATLIK}}                                                & \multicolumn{2}{c|}{\textbf{KANZI}}                                                 & \multicolumn{2}{c|}{\textbf{X264}}                                                  & \multicolumn{2}{c|}{\textbf{H2}}                                                           & \multicolumn{2}{c}{\textbf{JUMP3R}}                                                 \\ \cline{3-20} 
		\multirow{-2}{*}{\textbf{Workload}} & \multirow{-2}{*}{\textbf{Algorithm}} & \textbf{r}                         & \textbf{Mean (Std)}                             & \textbf{r}                         & \textbf{Mean (Std)}                             & \textbf{r}                         & \textbf{Mean (Std)}                            & \textbf{r}                         & \textbf{Mean (Std)}                             & \textbf{r}                         & \textbf{Mean (Std)}                            & \textbf{r}                         & \textbf{Mean (Std)}                            & \textbf{r}                         & \textbf{Mean (Std)}                            & \textbf{r}                         & \textbf{Mean (Std)}                                   & \textbf{r}                         & \textbf{Mean (Std)}                            \\ \hline
		& KGS                                  & 3                                  & 3.151 (0.079)                                   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{4.031 (1.052)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{5.861 (0.014)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.89 (0.166)}   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.914 (0.026)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.025 (0.992)} & \textbf{1}                         & \textbf{1.028 (0.313)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{26443.776 (1210.058)} & 3                                  & 2.599 (0.793)                                  \\
		& KGS-0.7                              & 2                                  & 3.14 (0.052)                                    & \textbf{1}                         & \textbf{4.09 (1.101)}                           & 3                                  & 5.88 (0.129)                                   & \textbf{1}                         & \textbf{1.95 (0.148)}                           & 2                                  & 0.916 (0.036)                                  & 2                                  & 1.189 (1.155)                                  & \textbf{1}                         & \textbf{1.029 (0.272)}                         & \textbf{1}                         & \textbf{26397.468 (857.114)}                          & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{2.421 (0.666)} \\
		& KGS-0.8                              & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{3.136 (0.033)}  & 2                                  & 4.484 (1.336)                                   & 2                                  & 5.876 (0.122)                                  & 2                                  & 1.976 (0.154)                                   & 3                                  & 0.937 (0.052)                                  & 2                                  & 1.34 (1.242)                                   & \textbf{1}                         & \textbf{1.045 (0.289)}                         & 2                                  & 25981.533 (1121.341)                                  & 2                                  & 2.449 (0.526)                                  \\
		\multirow{-4}{*}{workload-1}        & KGS-0.9                              & 3                                  & 3.186 (0.105)                                   & 2                                  & 4.592 (1.321)                                   & 1                                  & 5.869 (0.018)                                  & \textbf{1}                         & \textbf{1.976 (0.194)}                          & 3                                  & 0.949 (0.045)                                  & 3                                  & 1.952 (1.468)                                  & \cellcolor[HTML]{FFEFCA}\textbf{1} & \cellcolor[HTML]{FFEFCA}\textbf{1.027 (0.252)} & 2                                  & 25861.271 (1030.118)                                  & 3                                  & 2.823 (0.882)                                  \\ \hline
		& KGS                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.03 (0.0)}     & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.011 (0.003)}  & 3                                  & 1.945 (0.405)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.127 (0.064)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.341 (0.021)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.132 (0.029)} & \textbf{1}                         & \textbf{3.981 (0.949)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{18906.472 (512.334)}  & 2                                  & 0.854 (0.228)                                  \\
		& KGS-0.7                              & 2                                  & 0.03 (0.001)                                    & \textbf{1}                         & \textbf{0.012 (0.004)}                          & 3                                  & 1.815 (0.211)                                  & \textbf{1}                         & \textbf{1.156 (0.067)}                          & 2                                  & 1.345 (0.023)                                  & 2                                  & 0.133 (0.032)                                  & \textbf{1}                         & \textbf{4.007 (1.023)}                         & 2                                  & 18725.229 (629.802)                                   & \cellcolor[HTML]{FFCCC9}\textbf{1} & \cellcolor[HTML]{FFCCC9}\textbf{0.835 (0.184)} \\
		& KGS-0.8                              & 2                                  & 0.03 (0.001)                                    & 2                                  & 0.014 (0.005)                                   & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{1.761 (0.004)} & 2                                  & 1.17 (0.073)                                    & 3                                  & 1.363 (0.032)                                  & 2                                  & 0.139 (0.041)                                  & \textbf{1}                         & \textbf{4.008 (1.011)}                         & 3                                  & 18446.314 (938.093)                                   & 2                                  & 0.852 (0.196)                                  \\
		\multirow{-4}{*}{workload-2}        & KGS-0.9                              & 2                                  & 0.031 (0.003)                                   & 3                                  & 0.015 (0.005)                                   & 2                                  & 1.769 (0.089)                                  & 3                                  & 1.178 (0.072)                                   & 3                                  & 1.373 (0.037)                                  & 2                                  & 0.16 (0.045)                                   & \cellcolor[HTML]{FFEFCA}\textbf{1} & \cellcolor[HTML]{FFEFCA}\textbf{3.837 (0.753)} & 3                                  & 18398.95 (706.924)                                    & 2                                  & 0.979 (0.259)                                  \\ \hline
		& KGS                                  & 2                                  & 3.309 (0.018)                                   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.851 (0.897)}  & 2                                  & 0.615 (1.269)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.378 (0.008)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{4.204 (0.059)} & \textbf{1}                         & \textbf{0.298 (0.09)}                          & 2                                  & 1.439 (1.008)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{946.41 (48.138)}      & 2                                  & 1.295 (0.402)                                  \\
		& KGS-0.7                              & 2                                  & 3.307 (0.014)                                   & \textbf{1}                         & \textbf{4.057 (1.025)}                          & 2                                  & 0.67 (1.051)                                   & \textbf{1}                         & \textbf{0.381 (0.008)}                          & 2                                  & 4.214 (0.068)                                  & 2                                  & 0.314 (0.168)                                  & 2                                  & 1.577 (1.02)                                   & 2                                  & 930.52 (49.127)                                       & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{1.291 (0.371)} \\
		& KGS-0.8                              & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{3.307 (0.014)}  & 3                                  & 4.451 (1.325)                                   & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{0.603 (0.979)} & 2                                  & 0.383 (0.009)                                   & 3                                  & 4.25 (0.075)                                   & 2                                  & 0.31 (0.109)                                   & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{1.394 (0.348)} & 3                                  & 917.308 (46.955)                                      & 2                                  & 1.349 (0.5)                                    \\
		\multirow{-4}{*}{workload-3}        & KGS-0.9                              & 2                                  & 3.323 (0.03)                                    & 2                                  & 4.444 (1.264)                                   & 2                                  & 0.838 (1.146)                                  & 3                                  & 0.384 (0.008)                                   & 3                                  & 4.278 (0.105)                                  & \cellcolor[HTML]{FFEFCA}\textbf{1} & \cellcolor[HTML]{FFEFCA}\textbf{0.286 (0.068)} & 2                                  & 1.449 (0.427)                                  & 4                                  & 905.328 (50.681)                                      & 2                                  & 1.553 (0.504)                                  \\ \hline
		& KGS                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{7.132 (0.048)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{10.889 (2.631)} & \textbf{1}                         & \textbf{2.32 (0.199)}                          & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.629 (0.091)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.194 (0.025)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.397 (1.161)} & \textbf{1}                         & \textbf{1.752 (0.427)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1025.932 (55.874)}    & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.633 (0.089)} \\
		& KGS-0.7                              & 3                                  & 7.155 (0.141)                                   & \textbf{1}                         & \textbf{11.303 (3.072)}                         & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{2.32 (0.198)}  & 2                                  & 1.656 (0.099)                                   & 2                                  & 1.205 (0.026)                                  & \textbf{1}                         & \textbf{1.444 (1.168)}                         & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{1.728 (0.431)} & \textbf{1}                         & \textbf{1018.107 (63.207)}                            & 2                                  & 0.634 (0.087)                                  \\
		& KGS-0.8                              & 2                                  & 7.137 (0.057)                                   & 2                                  & 13.44 (3.701)                                   & \textbf{1}                         & \textbf{2.329 (0.283)}                         & 3                                  & 1.67 (0.091)                                    & 3                                  & 1.22 (0.027)                                   & 2                                  & 1.785 (1.937)                                  & \textbf{1}                         & \textbf{1.764 (0.466)}                         & 2                                  & 981.705 (97.968)                                      & 3                                  & 0.653 (0.106)                                  \\
		\multirow{-4}{*}{workload-4}        & KGS-0.9                              & 3                                  & 7.224 (0.185)                                   & 2                                  & 13.165 (4.09)                                   & \textbf{1}                         & \textbf{2.349 (0.179)}                         & 2                                  & 1.648 (0.082)                                   & 4                                  & 1.229 (0.036)                                  & 2                                  & 2.047 (1.531)                                  & \textbf{1}                         & \textbf{1.801 (0.465)}                         & 3                                  & 960.002 (97.84)                                       & 3                                  & 0.713 (0.133)                                  \\ \hline
		& KGS                                  & 2                                  & 33.495 (0.305)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{11.324 (3.145)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.215 (0.183)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.511 (0.022)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{2.412 (0.044)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.92 (0.646)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.529 (0.861)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{47795.98 (2476.631)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.063 (0.27)}  \\
		& KGS-0.7                              & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{33.463 (0.253)} & \textbf{1}                         & \textbf{12.298 (3.801)}                         & \textbf{1}                         & \textbf{3.279 (0.377)}                         & \textbf{1}                         & \textbf{0.519 (0.022)}                          & \textbf{1}                         & \textbf{2.415 (0.048)}                         & 2                                  & 1.001 (0.721)                                  & \textbf{1}                         & \textbf{3.578 (0.901)}                         & \textbf{1}                         & \textbf{47564.172 (2410.152)}                         & 2                                  & 1.084 (0.298)                                  \\
		& KGS-0.8                              & 2                                  & 33.464 (0.253)                                  & 2                                  & 12.912 (3.919)                                  & 2                                  & 3.325 (0.706)                                  & \textbf{1}                         & \textbf{0.522 (0.018)}                          & 2                                  & 2.462 (0.074)                                  & 3                                  & 1.247 (0.843)                                  & 2                                  & 3.737 (0.912)                                  & 2                                  & 47255.121 (2855.174)                                  & 3                                  & 1.181 (0.435)                                  \\
		\multirow{-4}{*}{workload-5}        & KGS-0.9                              & 2                                  & 33.669 (0.45)                                   & 3                                  & 13.4 (3.804)                                    & 1                                  & 3.283 (0.514)                                  & 2                                  & 0.523 (0.021)                                   & 2                                  & 2.474 (0.057)                                  & 3                                  & 1.723 (1.136)                                  & 2                                  & 3.7 (1.067)                                    & 2                                  & 47047.886 (3196.526)                                  & 3                                  & 1.327 (0.509)                                  \\ \hline
		& KGS                                  & 2                                  & 0.972 (0.004)                                   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.662 (0.434)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.363 (0.185)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.382 (0.014)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.173 (0.087)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.377 (0.178)} & \textbf{1}                         & \textbf{0.108 (0.017)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{48316.619 (468.084)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.296 (0.019)} \\
		& KGS-0.7                              & 2                                  & 0.972 (0.005)                                   & \textbf{1}                         & \textbf{1.785 (0.526)}                          & \textbf{1}                         & \textbf{1.375 (0.189)}                         & 2                                  & 0.386 (0.014)                                   & 2                                  & 3.209 (0.125)                                  & 2                                  & 0.459 (0.357)                                  & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{0.107 (0.019)} & 2                                  & 47360.297 (3163.938)                                  & 2                                  & 0.298 (0.022)                                  \\
		& KGS-0.8                              & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{0.972 (0.005)}  & 2                                  & 1.921 (0.569)                                   & 2                                  & 1.405 (0.23)                                   & 3                                  & 0.389 (0.013)                                   & 3                                  & 3.262 (0.152)                                  & 2                                  & 0.498 (0.388)                                  & \textbf{1}                         & \textbf{0.109 (0.018)}                         & 2                                  & 47428.4 (2383.591)                                    & 3                                  & 0.302 (0.026)                                  \\
		\multirow{-4}{*}{workload-6}        & KGS-0.9                              & 2                                  & 0.977 (0.009)                                   & 3                                  & 2.018 (0.499)                                   & 2                                  & 1.41 (0.309)                                   & 4                                  & 0.392 (0.013)                                   & 4                                  & 3.311 (0.15)                                   & 3                                  & 0.679 (0.446)                                  & \textbf{1}                         & \textbf{0.108 (0.018)}                         & 2                                  & 47312.967 (2769.771)                                  & 3                                  & 0.311 (0.031)                                  \\ \hline
		& KGS                                  & \textbf{1}                         & \textbf{0.196 (0.005)}                          & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.196 (0.014)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.275 (0.443)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{17.431 (2.813)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.14 (0.02)}   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.172 (0.07)}  & 2                                  & 0.665 (0.195)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{20086.443 (1268.046)} & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & 2                                  & 0.197 (0.004)                                   & \textbf{1}                         & \textbf{0.201 (0.02)}                           & \textbf{1}                         & \textbf{0.28 (0.21)}                           & 2                                  & 18.233 (3.344)                                  & 2                                  & 1.14 (0.02)                                    & 2                                  & 0.186 (0.081)                                  & \textbf{1}                         & \textbf{0.651 (0.19)}                          & 2                                  & 19740.264 (1637.713)                                  & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{0.196 (0.005)}  & 2                                  & 0.204 (0.016)                                   & \textbf{1}                         & \textbf{0.269 (0.194)}                         & \textbf{1}                         & \textbf{18.195 (3.302)}                         & 3                                  & 1.155 (0.029)                                  & 3                                  & 0.203 (0.096)                                  & 2                                  & 0.682 (0.432)                                  & 3                                  & 19145.558 (1980.915)                                  & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-7}        & KGS-0.9                              & 2                                  & 0.198 (0.005)                                   & 3                                  & 0.208 (0.02)                                    & \textbf{1}                         & \textbf{0.277 (0.212)}                         & \textbf{1}                         & \textbf{18.182 (3.314)}                         & 3                                  & 1.166 (0.037)                                  & 3                                  & 0.25 (0.118)                                   & \cellcolor[HTML]{FFEFCA}\textbf{1} & \cellcolor[HTML]{FFEFCA}\textbf{0.629 (0.144)} & 3                                  & 18844.881 (1944.615)                                  & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & 2                                  & 10.918 (0.041)                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{24.391 (6.316)} & \textbf{1}                         & \textbf{8.751 (0.025)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.038 (0.031)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{7.082 (0.163)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{2.554 (2.898)} & \textbf{1}                         & \textbf{0.148 (0.03)}                          & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{28148.776 (1869.212)} & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{10.913 (0.023)} & \textbf{1}                         & \textbf{25.491 (7.272)}                         & 2                                  & 8.752 (0.023)                                  & \textbf{1}                         & \textbf{1.049 (0.033)}                          & \textbf{1}                         & \textbf{7.113 (0.117)}                         & \textbf{1}                         & \textbf{2.609 (2.635)}                         & \textbf{1}                         & \textbf{0.151 (0.03)}                          & 2                                  & 27523.503 (2300.797)                                  & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 10.917 (0.025)                                  & 2                                  & 27.562 (8.184)                                  & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{8.748 (0.005)} & 3                                  & 1.061 (0.043)                                   & 2                                  & 7.216 (0.26)                                   & 2                                  & 3.42 (3.15)                                    & \textbf{1}                         & \textbf{0.149 (0.032)}                         & 3                                  & 26915.299 (2080.926)                                  & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-8}        & KGS-0.9                              & 2                                  & 10.946 (0.066)                                  & 2                                  & 28.999 (8.912)                                  & \textbf{1}                         & \textbf{8.752 (0.023)}                         & 2                                  & 1.058 (0.038)                                   & 3                                  & 7.237 (0.226)                                  & 2                                  & 4.04 (3.219)                                   & \cellcolor[HTML]{FFEFCA}\textbf{1} & \cellcolor[HTML]{FFEFCA}\textbf{0.145 (0.03)}  & 4                                  & 26456.794 (1945.466)                                  & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & 2                                  & 9.118 (0.364)                                   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{22.143 (6.448)} & \textbf{1}                         & \textbf{3.183 (0.005)}                         & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.48 (0.018)}   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.045 (0.008)} & 2                                  & 0.668 (0.555)                                  & \textbf{1}                         & \textbf{0.254 (0.034)}                         & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{9.098 (0.345)}  & \textbf{1}                         & \textbf{24.129 (7.586)}                         & \textbf{1}                         & \textbf{3.183 (0.005)}                         & 2                                  & 0.488 (0.016)                                   & 2                                  & 1.053 (0.018)                                  & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{0.654 (0.551)} & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{0.253 (0.034)} & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 9.164 (0.41)                                    & 2                                  & 25.968 (7.705)                                  & \cellcolor[HTML]{C0E3F8}\textbf{1} & \cellcolor[HTML]{C0E3F8}\textbf{3.183 (0.005)} & 3                                  & 0.493 (0.016)                                   & 3                                  & 1.066 (0.023)                                  & 3                                  & 0.79 (0.613)                                   & \textbf{1}                         & \textbf{0.267 (0.16)}                          & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-9}        & KGS-0.9                              & 2                                  & 9.344 (0.495)                                   & 3                                  & 26.495 (8.445)                                  & \textbf{1}                         & \textbf{3.184 (0.005)}                         & 2                                  & 0.489 (0.014)                                   & 4                                  & 1.072 (0.019)                                  & 3                                  & 1.152 (0.866)                                  & \textbf{1}                         & \textbf{0.253 (0.036)}                         & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                                 & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{5.312 (0.132)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{10.299 (2.475)} & \textbf{1}                         & \textbf{6.82 (0.235)}                          & 2                                  & 1.442 (0.008)                                   & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.115 (0.014)} & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & 2                                  & 5.319 (0.144)                                   & \textbf{1}                         & \textbf{11.626 (3.37)}                          & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{6.772 (0.22)}  & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{1.441 (0.009)}  & 2                                  & 1.121 (0.025)                                  & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 5.329 (0.166)                                   & 3                                  & 12.504 (3.937)                                  & 2                                  & 6.822 (0.233)                                  & 2                                  & 1.443 (0.01)                                    & 3                                  & 1.135 (0.033)                                  & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-10}       & KGS-0.9                              & 2                                  & 5.49 (0.335)                                    & 2                                  & 12.491 (3.373)                                  & \textbf{1}                         & \textbf{6.806 (0.249)}                         & 2                                  & 1.444 (0.011)                                   & 4                                  & 1.148 (0.033)                                  & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                                 & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{2.102 (0.035)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{2.626 (0.643)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{8.034 (0.847)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.447 (0.018)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{1.626 (0.028)} & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & 2                                  & 2.102 (0.036)                                   & \textbf{1}                         & \textbf{3.045 (0.954)}                          & 2                                  & 8.473 (1.394)                                  & \textbf{1}                         & \textbf{1.456 (0.019)}                          & \textbf{1}                         & \textbf{1.637 (0.047)}                         & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 2.106 (0.038)                                   & 2                                  & 3.217 (1.123)                                   & 2                                  & 8.16 (0.828)                                   & 2                                  & 1.458 (0.02)                                    & 2                                  & 1.679 (0.071)                                  & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-11}       & KGS-0.9                              & 2                                  & 2.13 (0.05)                                     & 3                                  & 3.245 (0.938)                                   & 2                                  & 8.186 (0.831)                                  & \textbf{1}                         & \textbf{1.457 (0.019)}                          & 3                                  & 1.691 (0.059)                                  & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                                 & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.499 (0.092)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{5.149 (1.346)}  & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{3.914 (0.114)} & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{0.488 (0.009)}  & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & 2                                  & 3.504 (0.097)                                   & \textbf{1}                         & \textbf{5.893 (1.841)}                          & \textbf{1}                         & \textbf{4.058 (1.515)}                         & 2                                  & 0.489 (0.009)                                   & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 3.507 (0.098)                                   & 2                                  & 6.343 (1.981)                                   & \textbf{1}                         & \textbf{3.95 (0.226)}                          & 3                                  & 0.491 (0.009)                                   & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-12}       & KGS-0.9                              & 2                                  & 3.58 (0.129)                                    & 3                                  & 6.426 (2.061)                                   & \textbf{1}                         & \textbf{3.918 (0.163)}                         & 3                                  & 0.493 (0.009)                                   & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                                 & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
		& KGS                                  & 2                                  & 2.53 (0.019)                                    & \cellcolor[HTML]{CBFECE}\textbf{1} & \cellcolor[HTML]{CBFECE}\textbf{2.926 (0.681)}  & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.7                              & \cellcolor[HTML]{FECDCD}\textbf{1} & \cellcolor[HTML]{FECDCD}\textbf{2.53 (0.019)}   & 2                                  & 3.1 (0.759)                                     & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		& KGS-0.8                              & 2                                  & 2.534 (0.022)                                   & 3                                  & 3.356 (0.92)                                    & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                               & \multicolumn{2}{c|}{}                                                                      & \multicolumn{2}{c}{}                                                                \\
		\multirow{-4}{*}{workload-13}       & KGS-0.9                              & 2                                  & 2.55 (0.025)                                    & 4                                  & 3.575 (0.969)                                   & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                           & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                          & \multicolumn{2}{c|}{\multirow{-4}{*}{N/A}}                                                 & \multicolumn{2}{c}{\multirow{-4}{*}{N/A}}                                           \\ \hline
	\end{tabular}	
}




==> tables/RQ4_sensitivity_comparison_summary.tex <==

	\begin{tabular}{c|cc|cc|cc|cc}
		\hline
		\multirow{2}{*}{System} & \multicolumn{2}{c|}{$\alpha$ = 0.6}             & \multicolumn{2}{c|}{$\alpha$ = 0.7}             & \multicolumn{2}{c|}{$\alpha$ = 0.8}             & \multicolumn{2}{c}{$\alpha$ = 0.9}              \\ \cline{2-9} 
		& \multicolumn{1}{c|}{$r$ = 1}       & perf. = best & \multicolumn{1}{c|}{$r$ = 1}       & perf. = best & \multicolumn{1}{c|}{$r$ = 1}       & perf. = best & \multicolumn{1}{c|}{$r$ = 1}       & perf. = best \\ \hline
		\textsc{lrzip}                   & \multicolumn{1}{c|}{6}           & 5            & \multicolumn{1}{c|}{4}           & 4            & \multicolumn{1}{c|}{4}           & 4            & \multicolumn{1}{c|}{0}           & 0            \\
		\textsc{xz}                      & \multicolumn{1}{c|}{13}          & 13           & \multicolumn{1}{c|}{12}          & 0            & \multicolumn{1}{c|}{0}           & 0            & \multicolumn{1}{c|}{0}           & 0            \\
		\textsc{z3}                      & \multicolumn{1}{c|}{9}           & 6            & \multicolumn{1}{c|}{7}           & 2            & \multicolumn{1}{c|}{7}           & 4            & \multicolumn{1}{c|}{8}           & 0            \\
		\textsc{dconvert}                & \multicolumn{1}{c|}{11}          & 11           & \multicolumn{1}{c|}{7}           & 1            & \multicolumn{1}{c|}{2}           & 0            & \multicolumn{1}{c|}{3}           & 0            \\
		\textsc{batlik}                  & \multicolumn{1}{c|}{11}          & 11           & \multicolumn{1}{c|}{3}           & 0            & \multicolumn{1}{c|}{0}           & 0            & \multicolumn{1}{c|}{0}           & 0            \\
		\textsc{kanzi}                   & \multicolumn{1}{c|}{8}           & 7            & \multicolumn{1}{c|}{3}           & 1            & \multicolumn{1}{c|}{0}           & 0            & \multicolumn{1}{c|}{1}           & 1            \\
		\textsc{x264}                    & \multicolumn{1}{c|}{7}           & 0            & \multicolumn{1}{c|}{8}           & 3            & \multicolumn{1}{c|}{7}           & 1            & \multicolumn{1}{c|}{7}           & 4            \\
		\textsc{h2}                      & \multicolumn{1}{c|}{8}           & 8            & \multicolumn{1}{c|}{3}           & 0            & \multicolumn{1}{c|}{0}           & 0            & \multicolumn{1}{c|}{0}           & 0            \\
		\textsc{jump3r}                  & \multicolumn{1}{c|}{3}           & 3            & \multicolumn{1}{c|}{3}           & 3            & \multicolumn{1}{c|}{0}           & 0            & \multicolumn{1}{c|}{0}           & 0            \\ \hline
		\textbf{Total}          & \multicolumn{1}{c|}{\textbf{76}} & \textbf{64}  & \multicolumn{1}{c|}{\textbf{50}} & \textbf{14}  & \multicolumn{1}{c|}{\textbf{20}} & \textbf{9}   & \multicolumn{1}{c|}{\textbf{19}} & \textbf{5}   \\ \hline
	\end{tabular}

==> tables/workload_mapping.tex <==



	\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
		\hline
		\textbf{Workload} & \textbf{\textsc{lrzip}}   & \textbf{\textsc{xz}}      & \textbf{\textsc{z3}}              & \textbf{\textsc{dconvert}} & \textbf{\textsc{batlik}}      & \textbf{\textsc{kanzi}}       & \textbf{\textsc{x264}}            & \textbf{\textsc{h2}}          & \textbf{\textsc{jump3r}}      \\ \hline
		$w_1$               & ambivert.wav.tar & ambivert.wav.tar & AUFNIRA\_z3             & jpeg-large        & corona               & ambivert             & Johnny\_short.y4m        & smallbank-1          & beethoven.wav        \\ \hline
		$w_2$               & artificl.tar     & artificl.tar     & LRA\_formula\_277   & jpeg-medium       & cranium              & artificl             & Netflix\_short.y4m       & smallbank-10         & dual-channel.wav     \\ \hline
		$w_3$               & deepfield.tar    & deepfield.tar    & QF\_AUFBV\_891           & jpeg-small        & cubus                & deepfield            & blue\_sky\_short.y4m     & tpcc-2               & helix.wav            \\ \hline
		$w_4$               & enwik8.tar       & enwik8.tar       & QF\_AUFLIA\_swap          & png-large         & flame                & enwik8               & pedestrian\_short.y4m    & tpcc-8               & single-channel.wav   \\ \hline
		$w_5$               & fannie.tar       & fannie.tar       & QF\_BV\_bench\_3176 & png-medium        & france               & fannie               & riverbed\_short.y4m      & voter-16             & speech.wav           \\ \hline
		$w_6$               & large.tar        & large.tar        & QF\_BV\_bench\_935  & png-small         & frisco               & large                & sd\_bridge\_short.y4m    & voter-2              & sweep.wav            \\ \hline
		$w_7$               & misc.tar         & misc.tar         & QF\_LIA\_tightrhombus    & psd-large         & jelly                & misc                 & sd\_city\_short.y4m      & ycsb-2400            & \multirow{7}{*}{N/A} \\ \cline{1-9}
		$w_8$               & silesia.tar      & silesia.tar      & QF\_LRA\_clocksynchro             & psd-medium        & karte                & silesia              & sd\_crew\_cif\_short.y4m & ycsb-600             &                      \\ \cline{1-9}
		$w_9$               & uiq-32.bin       & uiq-32.bin       & QF\_NRA\_hong             & psd-small         & mandelbrot           & vmlinux              & sintel\_short.y4m        & \multirow{5}{*}{N/A} &                      \\ \cline{1-8}
		$w_{10}$              & uiq2-16.bin      & uiq2-16.bin      & QF\_RDL\_orb08             & svg-large         & strawberry           & \multirow{4}{*}{N/A} & \multirow{4}{*}{N/A}     &                      &                      \\ \cline{1-6}
		$w_{11}$             & uiq2-4.bin       & uiq2-4.bin       & QF\_UFLIA\_xs           & svg-medium        & village              &                      &                          &                      &                      \\ \cline{1-6}
		$w_{12}$              & uiq2-8.bin       & uiq2-8.bin       & QF\_UF\_PEQ018              & svg-large         & \multirow{2}{*}{N/A} &                      &                          &                      &                      \\ \cline{1-5}
		$w_{13}$             & vmlinux-5.10.tar & vmlinux-5.10.tar & N/A                      & N/A               &                      &                      &                          &                      &                      \\ \hline
	\end{tabular}

